A Carbon-Cycle Based Stochastic Cellular Automata Climate Model

In this article a stochastic cellular automata model is examined, which has been developed to study a "small" world, where local changes may noticeably alter global characteristics. This is applied to a climate model, where global temperature is determined by an interplay between atmospheric carbon dioxide and carbon stored by plant life. The latter can be relased by forest fires, giving rise to significant changes of global conditions within short time.

==> macros.tex <==
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

\newcommand{\1}{\ensuremath 1\!\!1}
\renewcommand{\AA}{\ensuremath\mathcal{A}}

\renewcommand{\d}{\ensuremath\mathrm{d}}
\newcommand{\D}{\ensuremath\mathcal{D}}
\newcommand{\E}{\ensuremath\mathrm{e}}
\newcommand{\eps}{\ensuremath\varepsilon}
\newcommand{\Exp}[1]{\ensuremath\left< #1 \right>}
\newcommand{\fdg}{\ensuremath{\; \Big| \;}}
\newcommand{\GG}{\ensuremath\mathcal{G}}
\newcommand{\Grp}{\ensuremath\mathbb{G}}
\newcommand{\I}{\ensuremath \mathrm{i}}
\newcommand{\Int}{\ensuremath \mathrm{int\,}}
\newcommand{\NN}{\ensuremath\mathbb{N}}
\newcommand{\norm}[1]{\ensuremath\left\| #1 \right\|}
\newcommand{\OO}{\ensuremath\mathcal{O}}
\newcommand{\RR}{\ensuremath\mathbb{R}}

\newcommand{\feyn}[1]{\ensuremath #1\!\!/\!\,}
\newcommand{\Feyn}[1]{\ensuremath #1\!\!\!/\!\;}
\newcommand{\FeynSlash}[1]{\not \!\!#1}
\newcommand{\feynslash}[1]{\not \!#1}
\newcommand{\Four}[1]{\mathfrak{#1}} % obsolete
\newcommand{\II}{\mathrm{i}}  % obsolete
\newcommand{\LL}{\mathcal{L}}
\newcommand{\Matrix}[1]{\mathbf{#1}}
\newcommand{\SI}[1]{\hat{#1}}
\newcommand{\Tr}{\mathrm{Tr}}
\newcommand{\V}[1]{\boldsymbol{#1}}

\newcommand{\vk}{\V{k}}
\newcommand{\vp}{\V{p}}
\newcommand{\vq}{\V{q}}

\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bp}{{\bf p}}
\newcommand{\bk}{{\bf k}}
\newcommand{\bq}{{\bf q}}
\newcommand{\bA}{{\bf A}}
\newcommand{\p}{\partial}
\newcommand{\too}{\rightarrow}

\newcommand{\Ord}{\mathcal{O}}

\newcommand{\Zitat}[2]{{\flushright
  \parbox{12cm}{\textit{#1}}\\ \smallskip
  \parbox{8cm}{#2}\\ \medskip}}

\newcommand{\Example}[1]{\par
\noindent \rule{16cm}{0.1mm}\\[-11pt]
%\noindent \rule{16cm}{0.2mm}\\[-11pt]
\noindent \rule{16cm}{0.3mm} \par
\noindent \textsc{Example:} #1 \par
\noindent \rule{16cm}{0.3mm}\\[-11pt]
%\noindent \rule{16cm}{0.2mm}\\[-11pt]
\noindent \rule{16cm}{0.1mm} \par}
